Development of linear functional arithmetic and its applications to the solution of interval linear systems with constraints

The work is devoted to the construction of a new interval arithmetic which would combine algorithmic efficiency and high quality estimation of the ranges of expressions.

==> Title.tex <==
\newcommand{\tocsecindent}{\hspace{7mm}}

\begin{titlepage}

\begin{center}
{\small МИНИСТЕРСТВО НАУКИ И ВЫСШЕГО ОБРАЗОВАНИЯ РОССИЙСКОЙ ФЕДЕРАЦИИ} \\
\vspace{1em}
{\small ФЕДЕРАЛЬНОЕ ГОСУДАРСТВЕННОЕ АВТОНОМНОЕ ОБРАЗОВАТЕЛЬНОЕ УЧРЕЖДЕНИЕ ВЫСШЕГО ОБРАЗОВАНИЯ}\\
\vspace{1em}
{\small «НОВОСИБИРСКИЙ НАЦИОНАЛЬНЫЙ ИССЛЕДОВАТЕЛЬСКИЙ ГОСУДАРСТВЕННЫЙ УНИВЕРСИТЕТ» (НОВОСИБИРСКИЙ ГОСУДАРСТВЕННЫЙ УНИВЕРСИТЕТ, НГУ)} \\
\end{center}

\vspace{1.5em}
\raggedright{\small Факультет \qquad \qquad Механико-математический факультет}\\*
\vspace{0.8em}
\raggedright{\small Кафедра \; \; \; \quad \qquad Математического моделирования} \\*
\vspace{1.5em}
\raggedright{\small Направление подготовки \qquad Прикладная математика и информатика}\\*
\vspace{1.5em}

\begin{center}
{\textbf{\small ВЫПУСКНАЯ КВАЛИФИКАЦИОННАЯ РАБОТА БАКАЛАВРА}} \\
\vspace{0.8em}
{\small Скорика Дмитрия Александровича}\\
\end{center}

\vspace{0.6em}
\begin{center}
{\small Тема работы: Разработка линейной функциональной арифметики и её приложения к решению интервальных линейных систем со связями}\\*
\end{center}
\vspace{2cm}

\begin{small}
	\begin{tabular}{m{8.5cm} l}
	
		\textbf{<<К защите допущен>>} & \textbf{Научный руководитель} \\ \vspace{1mm}
		
		Заведующий кафедрой, & Д. ф.-м. н., \\ \vspace{1mm}
		
		д. ф.-м. н., проф. & в. н. с. ФИЦ ИВТ \\ \vspace{1mm}
		
		\underline{ Шарый С. П. } / \underline{\phantom{ПодписьПодпись}} & \underline{ Шарый С. П. } / \underline{\phantom{ПодписьПодпись}} \\
		
		\footnotesize{(Фамилия И. О.)} \hspace{1cm} \footnotesize{(Подпись)} & \footnotesize{(Фамилия И. О.)} \hspace{1cm} \footnotesize{(Подпись)} \\ \vspace{1mm}
		
		<<\,.\,.\,.\,>>\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,2020г. & <<\,.\,.\,.\,>>\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,.\,2020г.

	\end{tabular}
\end{small}

\vspace{3.2cm}
\raggedright{\small \ \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad Дата защиты:  \makebox[0.07\textwidth][l]{«\dotfill»}\makebox[0.3\textwidth][l]{\dotfill 2020 г.}} \\
\vspace{0.5cm}
\begin{center}
{\small Новосибирск, 2020} 
\end{center}

\thispagestyle{empty}
\end{titlepage}
